Chance-Constrained Set Covering with Wasserstein Ambiguity

We study a generalized distributionally robust chance-constrained set covering problem (DRC) with a Wasserstein ambiguity set, where both decisions and uncertainty are binary-valued. We establish the NP-hardness of DRC and recast it as a two-stage stochastic program, which facilitates decomposition algorithms. Furthermore, we derive two families of valid inequalities. The first family targets the hypograph of a "shifted" submodular function, which is associated with each scenario of the two-stage reformulation. We show that the valid inequalities give a complete description of the convex hull of the hypograph. The second family mixes inequalities across multiple scenarios and gains further strength via lifting. Our numerical experiments demonstrate the reliability of the DRC model and the effectiveness of our proposed reformulation and valid inequalities.

==> figs2/bench_vs_xie.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{tabular}{rrrr|rr|rrr}
  \toprule
                                       &        &       &            & \multicolumn{2}{c}{\texttt{bin}} & \multicolumn{2}{c}{\texttt{cont}} \\
  % \cmidrule{5-8}
  \(n\)                                & \(I\)  & \(N\) & \(\delta\) & Optval                           & Time  & Optval   & Time           \\
  \midrule
  20                                   & 10     & 50    & 0.01       & 136.00                           & 1.31  & 270.40   & 8.13           \\
                                       &        &       & 0.05       & 159.40                           & 0.94  & 557.40   & 7.02           \\
                                       &        &       & 0.1        & 203.40                           & 0.62  & INF      & 0.55           \\
                                       &        & 100   & 0.01       & 115.40                           & 2.38  & 239.80   & 15.58          \\
                                       &        &       & 0.05       & 128.80                           & 1.39  & 552.40   & 18.00          \\
                                       &        &       & 0.1        & 210.60                           & 1.16  & 1,020.00 & 1.66           \\
                                       & 25     & 50    & 0.01       & 200.20                           & 2.32  & 365.20   & 15.99          \\
                                       &        &       & 0.05       & 216.20                           & 1.50  & 615.75   & 9.96           \\
                                       &        &       & 0.1        & 258.00                           & 0.99  & INF      & 0.67           \\
                                       &        & 100   & 0.01       & 213.80                           & 5.50  & 409.20   & 49.20          \\
                                       &        &       & 0.05       & 233.80                           & 2.98  & 841.75   & 8.17           \\
                                       &        &       & 0.1        & 304.80                           & 1.83  & INF      & 1.16           \\
  30                                   & 10     & 50    & 0.01       & 150.20                           & 11.24 & 236.60   & 109.86         \\
                                       &        &       & 0.05       & 161.60                           & 5.83  & 404.00   & 109.56         \\
                                       &        &       & 0.1        & 204.20                           & 1.63  & 752.60   & 44.02          \\
                                       &        & 100   & 0.01       & 147.00                           & 13.62 & 255.20   & 191.69         \\
                                       &        &       & 0.05       & 162.60                           & 5.58  & 459.20   & 108.07         \\
                                       &        &       & 0.1        & 223.60                           & 2.32  & 959.20   & 33.22          \\
                                       & 25     & 50    & 0.01       & 205.60                           & 19.16 & 322.60   & 177.63         \\
                                       &        &       & 0.05       & 226.20                           & 8.46  & 544.80   & 96.73          \\
                                       &        &       & 0.1        & 252.80                           & 3.33  & 1,253.67 & 7.09           \\
                                       &        & 100   & 0.01       & 173.20                           & 23.38 & 305.80   & 588.23         \\
                                       &        &       & 0.05       & 199.40                           & 10.16 & 579.80   & 282.40         \\
                                       &        &       & 0.1        & 261.40                           & 3.68  & 1,201.33 & 24.23          \\
  \midrule
  \multicolumn{4}{c|}{Average} & 197.84 & 5.47  & 578.41     & 79.53                                                                \\
  \bottomrule
\end{tabular}


==> figs2/mono_vs_2stg.tex <==
\begin{tabular}{llll|rrr|rrr}
\toprule
        &       &       &             & \multicolumn{3}{c}{\texttt{1-Stg}} & \multicolumn{3}{c}{\texttt{2-Stg}}                   \\
  \(n\) & \(I\) & \(N\) & \(\delta\)  & Optval                             & Time    & Gap \(\%\) & Optval & Time    & Gap \(\%\) \\
\midrule
100     & 150   & 100   & 0.2         & 239.0                              & 47.35   & 0.00       & 239.0  & 5.49    & 0.0        \\
        &       &       & 0.4         & 1619.0                             & 283.79  & 0.00       & 1619.0 & 23.42   & 0.0        \\
        &       & 300   & 0.2         & 413.0                              & 3600.02 & 5.08       & 413.0  & 467.97  & 0.0        \\
        &       &       & 0.4         & 1864.0                             & 3600.01 & 1.56       & 1864.0 & 366.69  & 0.0        \\
        & 300   & 100   & 0.2         & 285.0                              & 155.00  & 0.00       & 285.0  & 8.32    & 0.0        \\
        &       &       & 0.4         & 1495.0                             & 514.63  & 0.00       & 1495.0 & 17.96   & 0.0        \\
        &       & 300   & 0.2         & 357.0                              & 1414.82 & 0.00       & 357.0  & 54.77   & 0.0        \\
        &       &       & 0.4         & 1746.0                             & 3600.02 & 1.78       & 1746.0 & 285.58  & 0.0        \\
200     & 150   & 100   & 0.2         & 125.0                              & 45.94   & 0.00       & 125.0  & 6.88    & 0.0        \\
        &       &       & 0.4         & 815.0                              & 1117.46 & 0.00       & 815.0  & 64.69   & 0.0        \\
        &       & 300   & 0.2         & 180.0                              & 929.67  & 0.00       & 180.0  & 34.73   & 0.0        \\
        &       &       & 0.4         & 791.0                              & 3600.02 & 2.02       & 791.0  & 550.72  & 0.0        \\
        & 300   & 100   & 0.2         & 173.0                              & 207.36  & 0.00       & 173.0  & 15.07   & 0.0        \\
        &       &       & 0.4         & 729.0                              & 505.21  & 0.00       & 729.0  & 14.54   & 0.0        \\
        &       & 300   & 0.2         & 191.0                              & 3600.08 & 6.28       & 191.0  & 394.36  & 0.0        \\
        &       &       & 0.4         & 880.0                              & 3600.09 & 2.95       & 880.0  & 3600.00 & 0.8        \\
\bottomrule
\end{tabular}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> tbls/bench-effi.tex <==
\begin{tabular}{@{}lllll|ll|ll|ll@{}}
\toprule
    &     &     &          &            & \multicolumn{2}{c}{\texttt{\(2\)-Stg}} & \multicolumn{2}{c}{\texttt{+single}} & \multicolumn{2}{c}{\texttt{+cross}}            \\
$n$ & $I$ & $N$ & $\delta$ & $\epsilon$ & time                      & gap (\%)                    & time   & gap (\%) & time   & gap (\%) \\
\midrule
40  & 35  & 100 & 0.05     & 0.1        & 514.3                     & 0.0                         & 245.4  & 0.0      & 41.7   & 0.0      \\
    &     &     &          & 0.2        & 1510.8                    & 0.0                         & 2236.3 & 6.4 (2)  & 123.5  & 0.0      \\
    &     &     & 0.10     & 0.1        & 13.4                      & 0.0                         & 17.6   & 0.0      & 9.7    & 0.0      \\
    &     &     &          & 0.2        & 647.9                     & 0.0                         & 354.5  & 0.0      & 125.0  & 0.0      \\
    &     &     & 0.20     & 0.1        & 3.6                       & 0.0                         & 12.0   & 0.0      & 8.8    & 0.0      \\
    &     &     &          & 0.2        & 26.6                      & 0.0                         & 37.2   & 0.0      & 14.6   & 0.0      \\
    & 45  & 100 & 0.05     & 0.1        & 238.2                     & 0.0                         & 170.9  & 0.0      & 43.6   & 0.0      \\
    &     &     &          & 0.2        & 1025.3                    & 3.3 (1)                     & 1302.8 & 4.7 (1)  & 151.6  & 0.0      \\
    &     &     & 0.10     & 0.1        & 11.3                      & 0.0                         & 20.5   & 0.0      & 10.7   & 0.0      \\
    &     &     &          & 0.2        & 391.6                     & 0.0                         & 263.9  & 0.0      & 73.2   & 0.0      \\
    &     &     & 0.20     & 0.1        & 4.3                       & 0.0                         & 13.6   & 0.0      & 10.3   & 0.0      \\
    &     &     &          & 0.2        & 25.6                      & 0.0                         & 38.3   & 0.0      & 19.1   & 0.0      \\
50  & 35  & 100 & 0.05     & 0.1        & 1821.6                    & 10.3 (2)                    & 1402.1 & 5.6 (1)  & 807.8  & 0.6 (1)  \\
    &     &     &          & 0.2        & 2232.2                    & 21.3 (3)                    & 2358.9 & 22.7 (2) & 1163.6 & 2.9 (1)  \\
    &     &     & 0.10     & 0.1        & 736.9                     & 0.8  (1)                    & 445.1  & 0.0      & 97.4   & 0.0      \\
    &     &     &          & 0.2        & 1824.0                    & 15.1 (2)                    & 1580.9 & 5.9 (1)  & 895.8  & 3.4 (1)  \\
    &     &     & 0.20     & 0.1        & 6.3                       & 0.0                         & 19.5   & 0.0      & 11.4   & 0.0      \\
    &     &     &          & 0.2        & 739.5                     & 0.0                         & 232.0  & 0.0      & 60.2   & 0.0      \\
    & 45  & 100 & 0.05     & 0.1        & 2614.8                    & 11.0 (3)                    & 2303.4 & 3.9 (2)  & 270.9  & 0.0      \\
    &     &     &          & 0.2        & 3324.5                    & 30.9 (4)                    & 3600.0 & 35.9 (5) & 1743.8 & 0.6 (1)  \\
    &     &     & 0.10     & 0.1        & 70.5                      & 0.0                         & 66.6   & 0.0      & 21.8   & 0.0      \\
    &     &     &          & 0.2        & 2868.4                    & 18.4 (3)                    & 2660.3 & 8.2 (3)  & 560.0  & 0.0      \\
    &     &     & 0.20     & 0.1        & 6.0                       & 0.0                         & 18.6   & 0.0      & 11.6   & 0.0      \\
    &     &     &          & 0.2        & 219.8                     & 0.0                         & 110.1  & 0.0      & 46.6   & 0.0      \\
\bottomrule
\end{tabular}


==> tbls/bench_raw.tex <==
\begin{tabular}{lllllrlrlrl}
\toprule
   &    &     &      &      & \multicolumn{2}{l}{2-Stg} & \multicolumn{2}{l}{+single} & \multicolumn{2}{l}{+cross} \\
   &    &     &      &      &    time & gap (%) &    time & gap (%) &    time & gap (%) \\
$n$ & $I$ & $N$ & $\delta$ & $\epsilon$ &         &         &         &         &         &         \\
\midrule
60 & 70 & 50  & 0.05 & 0.05 &  1498.0 &       2 &    63.5 &       0 &    38.0 &       0 \\
   &    &     &      & 0.10 &  3057.4 &    30.1 &  3009.7 &    19.5 &  1447.3 &     0.6 \\
   &    &     & 0.10 & 0.05 &     5.3 &       0 &    11.8 &       0 &     8.7 &       0 \\
   &    &     &      & 0.10 &   836.3 &     2.9 &   722.8 &       0 &   188.8 &       0 \\
   &    &     & 0.20 & 0.05 &     1.6 &     INF &     9.1 &     INF &     6.4 &     INF \\
   &    &     &      & 0.10 &     5.7 &       0 &    12.1 &       0 &     8.6 &       0 \\
   &    &     & 0.30 & 0.05 &     1.1 &     INF &     7.4 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &     3.8 &       0 &    11.7 &       0 &     8.7 &       0 \\
   &    & 100 & 0.05 & 0.05 &   968.7 &       2 &   671.5 &       0 &   247.8 &       0 \\
   &    &     &      & 0.10 &  3600.0 &    43.6 &  3600.0 &    29.9 &  2103.2 &     6.5 \\
   &    &     & 0.10 & 0.05 &    10.8 &       0 &    25.6 &       0 &    18.7 &       0 \\
   &    &     &      & 0.10 &  1903.4 &     2.9 &   990.7 &     0.7 &   264.7 &       0 \\
   &    &     & 0.20 & 0.05 &     2.5 &     INF &    18.4 &     INF &    13.9 &     INF \\
   &    &     &      & 0.10 &    13.5 &       0 &    32.2 &       0 &    18.5 &       0 \\
   &    &     & 0.30 & 0.05 &     2.0 &     INF &    14.8 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &     8.0 &       0 &    26.6 &       0 &    17.4 &       0 \\
   &    & 200 & 0.05 & 0.05 &   432.4 &       0 &   326.5 &       0 &    81.6 &       0 \\
   &    &     &      & 0.10 &  3600.0 &    44.7 &  3600.0 &    32.8 &  3428.5 &     7.7 \\
   &    &     & 0.10 & 0.05 &    14.2 &       0 &    47.8 &       0 &    34.2 &       0 \\
   &    &     &      & 0.10 &  1731.0 &     0.6 &   745.4 &       0 &   152.7 &       0 \\
   &    &     & 0.20 & 0.05 &     4.3 &     INF &    35.5 &     INF &    31.5 &     INF \\
   &    &     &      & 0.10 &    25.2 &       0 &    67.3 &       0 &    38.1 &       0 \\
   &    &     & 0.30 & 0.05 &     3.4 &     INF &    30.0 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &    13.4 &       0 &    50.1 &       0 &    39.5 &       0 \\
   & 90 & 50  & 0.05 & 0.05 &  2333.7 &     8.2 &    70.1 &       0 &    31.0 &       0 \\
   &    &     &      & 0.10 &  3600.3 &      44 &  3600.0 &    30.3 &  1829.0 &       0 \\
   &    &     & 0.10 & 0.05 &    10.4 &       0 &    14.2 &       0 &    10.6 &       0 \\
   &    &     &      & 0.10 &  3328.5 &       9 &   905.8 &       0 &   184.5 &       0 \\
   &    &     & 0.20 & 0.05 &     1.8 &     INF &     9.0 &     INF &     6.6 &     INF \\
   &    &     &      & 0.10 &     9.1 &       0 &    15.1 &       0 &    11.0 &       0 \\
   &    &     & 0.30 & 0.05 &     1.2 &     INF &     7.2 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &     4.5 &       0 &    11.9 &       0 &     9.2 &       0 \\
   &    & 100 & 0.05 & 0.05 &  2696.9 &       8 &  1159.9 &     2.1 &   307.0 &       0 \\
   &    &     &      & 0.10 &  3600.0 &    48.1 &  3600.1 &      35 &  2594.6 &     8.5 \\
   &    &     & 0.10 & 0.05 &    18.0 &       0 &    34.0 &       0 &    22.3 &       0 \\
   &    &     &      & 0.10 &  2440.3 &     4.8 &  1717.0 &     1.7 &   544.9 &     0.7 \\
   &    &     & 0.20 & 0.05 &     2.7 &     INF &    18.1 &     INF &    13.9 &     INF \\
   &    &     &      & 0.10 &    24.0 &       0 &    53.4 &       0 &    27.4 &       0 \\
   &    &     & 0.30 & 0.05 &     2.1 &     INF &    15.0 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &    11.6 &       0 &    33.1 &       0 &    20.9 &       0 \\
   &    & 200 & 0.05 & 0.05 &  2044.0 &     2.1 &   809.0 &       0 &   105.8 &       0 \\
   &    &     &      & 0.10 &  3600.0 &    48.8 &  3600.9 &    36.4 &  3566.4 &      13 \\
   &    &     & 0.10 & 0.05 &    22.9 &       0 &    63.3 &       0 &    41.1 &       0 \\
   &    &     &      & 0.10 &  2930.7 &     6.3 &  2457.6 &     2.8 &   461.4 &       0 \\
   &    &     & 0.20 & 0.05 &     5.0 &     INF &    36.6 &     INF &    26.9 &     INF \\
   &    &     &      & 0.10 &    48.5 &       0 &    95.8 &       0 &    50.0 &       0 \\
   &    &     & 0.30 & 0.05 &     3.7 &     INF &    29.1 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &    23.3 &       0 &    74.4 &       0 &    46.3 &       0 \\
80 & 70 & 50  & 0.05 & 0.05 &  3600.0 &    42.7 &  3088.9 &    10.8 &  2333.8 &     6.6 \\
   &    &     &      & 0.10 &  3600.0 &    65.2 &  3600.1 &    51.2 &  3600.0 &    23.4 \\
   &    &     & 0.10 & 0.05 &    27.1 &       0 &    27.9 &       0 &    18.6 &       0 \\
   &    &     &      & 0.10 &  3600.2 &      35 &  3431.0 &    10.9 &  2622.2 &     7.1 \\
   &    &     & 0.20 & 0.05 &     7.2 &       0 &    17.8 &       0 &    12.7 &       0 \\
   &    &     &      & 0.10 &    23.7 &       0 &    31.4 &       0 &    20.2 &       0 \\
   &    &     & 0.30 & 0.05 &     1.7 &     INF &    14.1 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &     7.5 &       0 &    20.6 &       0 &    13.9 &       0 \\
   &    & 100 & 0.05 & 0.05 &  3600.0 &    30.6 &  3305.9 &     9.8 &  2528.1 &     6.1 \\
   &    &     &      & 0.10 &  3600.0 &      65 &  3600.2 &    51.1 &  3600.0 &    26.1 \\
   &    &     & 0.10 & 0.05 &   225.6 &       0 &   102.0 &       0 &    53.8 &       0 \\
   &    &     &      & 0.10 &  3600.1 &    29.8 &  3600.0 &    16.6 &  2941.8 &     9.2 \\
   &    &     & 0.20 & 0.05 &     7.4 &       0 &    33.4 &       0 &    24.6 &       0 \\
   &    &     &      & 0.10 &   415.2 &       0 &   234.7 &       0 &    60.2 &       0 \\
   &    &     & 0.30 & 0.05 &     2.9 &     INF &    29.3 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &    23.8 &       0 &    60.8 &       0 &    35.5 &       0 \\
   &    & 200 & 0.05 & 0.05 &  3600.0 &    31.3 &  3600.0 &    21.2 &  3600.0 &    12.9 \\
   &    &     &      & 0.10 &  3600.1 &     INF &  3600.4 &    54.3 &  3600.3 &    35.4 \\
   &    &     & 0.10 & 0.05 &   193.8 &       0 &   165.2 &       0 &    78.3 &       0 \\
   &    &     &      & 0.10 &  3600.0 &    31.3 &  3600.2 &    22.1 &  3600.0 &    12.9 \\
   &    &     & 0.20 & 0.05 &    15.2 &       0 &    71.2 &       0 &    56.2 &       0 \\
   &    &     &      & 0.10 &   180.7 &       0 &   200.7 &       0 &    97.5 &       0 \\
   &    &     & 0.30 & 0.05 &     5.8 &     INF &    58.6 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &    46.0 &       0 &   119.7 &       0 &    83.9 &       0 \\
   & 90 & 50  & 0.05 & 0.05 &  3600.1 &    39.6 &  3126.5 &     5.2 &  2203.9 &     1.1 \\
   &    &     &      & 0.10 &  3600.0 &    64.1 &  3600.1 &    52.1 &  3600.0 &    22.5 \\
   &    &     & 0.10 & 0.05 &    57.0 &       0 &    30.3 &       0 &    19.3 &       0 \\
   &    &     &      & 0.10 &  3600.1 &    35.5 &  3600.0 &    16.1 &  3255.6 &     8.2 \\
   &    &     & 0.20 & 0.05 &     6.5 &       0 &    17.0 &       0 &    12.6 &       0 \\
   &    &     &      & 0.10 &    44.0 &       0 &    32.6 &       0 &    21.6 &       0 \\
   &    &     & 0.30 & 0.05 &     2.0 &     INF &    14.9 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &     9.2 &       0 &    19.5 &       0 &    14.7 &       0 \\
   &    & 100 & 0.05 & 0.05 &  3600.0 &    30.8 &  3579.4 &    10.4 &  3197.5 &     7.4 \\
   &    &     &      & 0.10 &  3600.3 &    65.5 &  3601.0 &      52 &  3600.3 &    27.1 \\
   &    &     & 0.10 & 0.05 &    46.6 &       0 &    50.8 &       0 &    35.1 &       0 \\
   &    &     &      & 0.10 &  3600.0 &    27.1 &  3600.0 &    15.2 &  3241.2 &     7.5 \\
   &    &     & 0.20 & 0.05 &     7.2 &       0 &    31.9 &       0 &    23.9 &       0 \\
   &    &     &      & 0.10 &    95.5 &       0 &    70.5 &       0 &    38.1 &       0 \\
   &    &     & 0.30 & 0.05 &     3.1 &     INF &    28.7 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &    24.4 &       0 &    59.2 &       0 &    34.1 &       0 \\
   &    & 200 & 0.05 & 0.05 &  3600.0 &    23.3 &  3600.0 &    14.5 &  2141.8 &     3.2 \\
   &    &     &      & 0.10 &  3600.2 &     INF &  3601.2 &    51.7 &  3600.0 &    30.1 \\
   &    &     & 0.10 & 0.05 &   110.8 &       0 &   163.7 &       0 &    98.2 &       0 \\
   &    &     &      & 0.10 &  3600.0 &    30.3 &  3600.0 &    17.6 &  3600.0 &     6.3 \\
   &    &     & 0.20 & 0.05 &    14.3 &       0 &    69.9 &       0 &    47.9 &       0 \\
   &    &     &      & 0.10 &   856.0 &     0.1 &   787.7 &       0 &   136.4 &       0 \\
   &    &     & 0.30 & 0.05 &     6.0 &     INF &    56.6 &     INF &     0.0 &     INF \\
   &    &     &      & 0.10 &   123.2 &       0 &   278.2 &       0 &   110.7 &       0 \\
\bottomrule
\end{tabular}

